A speed preserving Hilbert gradient flow for generalized integral Menger curvature

We establish long-time existence for a projected Sobolev gradient flow of generalized integral Menger curvature in the Hilbert case, and provide $C^{1,1}$-bounds in time for the solution that only depend on the initial curve. The self-avoidance property of integral Menger curvature guarantees that the knot class of the initial curve is preserved under the flow, and the projection ensures that each curve along the flow is parametrized with the same speed as the initial configuration. Finally, we describe how to simulate this flow numerically with substantially higher efficiency than in the corresponding numerical $L^2$ gradient descent or other optimization methods.

==> Numerics/LineSearch_pdf.tex <==
%%
%% Creator: Mathematica 12.0.0 for Mac OS X x86 (64-bit) (April 7, 2019)
%% Export script by Henrik Schumacher, 2014
%% Abstracted from PDF/EPS/PS + LaTeX output extension by Johan Engelen, 2010
%% Accompanies image file 'LineSearch.pdf' 
%%
%% To include the image in your LaTeX document, write
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics{<filename>.pdf}
%% To scale the image, write
%%   \def\svgwidth{<desired width>}
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics[width=<desired width>]{<filename>.pdf}
%%
%% Images with a different path to the parent latex file can
%% be accessed by specifying
%%   \graphicspath{{<path to file>/}}
\begingroup%
  \makeatletter%
  \providecommand\color[2][]{%
    \errmessage{(Inkscape) Color is used for the text in Inkscape, but the package 'color.sty' is not loaded}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\transparent[1]{%
    \errmessage{(Inkscape) Transparency is used (non-zero) for the text in Inkscape, but the package 'transparent.sty' is not loaded}%
    \renewcommand\transparent[1]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \ifx\svgwidth\undefined%
    \setlength{\unitlength}{360bp}%
    \ifx\svgscale\undefined%
      \relax%
    \else%
      \setlength{\unitlength}{\unitlength * \real{\svgscale}}%
    \fi%
  \else%
    \setlength{\unitlength}{\svgwidth}%
  \fi%
  \global\let\svgwidth\undefined%
  \global\let\svgscale\undefined%
  \makeatother%
  \begin{picture}(1,0.9984)%
    \put(0,0){\includegraphics[width=\unitlength]{LineSearch.pdf}}%
    \put(0.064444444,0.37475556){\makebox(0,0)[cb]{\smash{$\varphi(0)$}}}%
    \put(0.73111111,0.68586667){\makebox(0,0)[cb]{\smash{$\tau \mapsto \varphi(\tau)$}}}%
    \put(0.46444444,0.39253333){\makebox(0,0)[cb]{\smash{$\tau \mapsto \varphi(0) + \sigma \, \tau \, \varphi'(0)$}}}%
    \put(0.064444444,0.86364444){\makebox(0,0)[cb]{\smash{$\varphi$}}}%
    \put(0.90888889,0.063644444){\makebox(0,0)[cb]{\smash{$\tau$}}}%
  \end{picture}%
\endgroup%

==> Numerics/RestoringFeasibility_pdf.tex <==
%%
%% Creator: Mathematica 12.0.0 for Mac OS X x86 (64-bit) (April 7, 2019)
%% Export script by Henrik Schumacher, 2014
%% Abstracted from PDF/EPS/PS + LaTeX output extension by Johan Engelen, 2010
%% Accompanies image file 'RestoringFeasibility.pdf' 
%%
%% To include the image in your LaTeX document, write
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics{<filename>.pdf}
%% To scale the image, write
%%   \def\svgwidth{<desired width>}
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics[width=<desired width>]{<filename>.pdf}
%%
%% Images with a different path to the parent latex file can
%% be accessed by specifying
%%   \graphicspath{{<path to file>/}}
\begingroup%
  \makeatletter%
  \providecommand\color[2][]{%
    \errmessage{(Inkscape) Color is used for the text in Inkscape, but the package 'color.sty' is not loaded}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\transparent[1]{%
    \errmessage{(Inkscape) Transparency is used (non-zero) for the text in Inkscape, but the package 'transparent.sty' is not loaded}%
    \renewcommand\transparent[1]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \ifx\svgwidth\undefined%
    \setlength{\unitlength}{360bp}%
    \ifx\svgscale\undefined%
      \relax%
    \else%
      \setlength{\unitlength}{\unitlength * \real{\svgscale}}%
    \fi%
  \else%
    \setlength{\unitlength}{\svgwidth}%
  \fi%
  \global\let\svgwidth\undefined%
  \global\let\svgscale\undefined%
  \makeatother%
  \begin{picture}(1,0.9984)%
    \put(0,0){\includegraphics[width=\unitlength]{RestoringFeasibility.pdf}}%
    \put(0.42,0.66364444){\makebox(0,0)[cb]{\smash{$P(t)$}}}%
    \put(0.64222222,0.66364444){\makebox(0,0)[cb]{\smash{$\dot{P}(t)$}}}%
    \put(0.97555556,0.69475556){\makebox(0,0)[cb]{\smash{$Q_0(\tau)$}}}%
    \put(0.97555556,0.46364444){\makebox(0,0)[cb]{\smash{$Q_\infty(\tau)$}}}%
    \put(0.10888889,0.70808889){\makebox(0,0)[cb]{\smash{$\ker(D\SIGMA_\Triangulation(P(t)))$}}}%
    \put(0.73111111,0.90808889){\makebox(0,0)[cb]{\smash{$\ker(D\SIGMA_\Triangulation(P(t)))^\perp$}}}%
    \put(0.77555556,0.17475556){\makebox(0,0)[cb]{\smash{$\{\SIGMA_\Triangulation = 0\}$}}}%
  \end{picture}%
\endgroup%
